Enhancing Speckle Statistics for Imaging inside Scattering Media

We exploit memory effect speckle correlations for the imaging of incoherent linear (single-photon) fluorescent sources behind scattering tissue. While memory effect-based imaging techniques have been heavily studied in the past, for thick scattering layers and complex illumination patterns these correlations are weak, limiting the practice applicability of the idea. In this work, we introduce a Spatial Light Modulator (SLM) between the tissue sample and the imaging sensor and capture multiple modulations of the speckle pattern. We show that by correctly designing the modulation pattern and the reconstruction algorithm we can greatly enhance statistical correlations in the data. We exploit this to demonstrate the reconstruction of mega-pixel wide fluorescent patterns behind scattering tissue.

==> algorithm.tex <==
\begin{algorithm}[t]
	\caption{Reconstruction pipeline for {\AlgName}.}
	\label{alg:pipeline}
	1. Capture interference signal $I_t$ as discussed in \secref{sec:exp}.\ref{sec:interf}\\
    2. Calculate local correlations, correct phase and average local correlations, using \eqref{eq:local-avg-corr}.\\
    3. Solve for latent image explaining local correlations, \eqref{eq:obj}.
\end{algorithm} 

==> figure/compare_S_autocorrelation_TI_only.tex <==
%\newcommand*{\doublec}[1]{%
%    \multicolumn{2}{c}{ \shifttext{-2em}{#1}}
%}

\begin{figure}[t]
\centering
%\hspace{-2em}
\begin{tabular}{PP@{\hskip 1.8em}PP}
%\comparemethodssp{./figure/compare/collisionfree_fewer_A} \\
%\comparemethodssp{./figure/compare/collisionfree_A} \\
\comparecorrectionmix{./figure/compare/collisionfree_fewer_A}{./figure/compare/collisionfree_A}\\
\doublec{(a) w/o correction} & \doublec{(b) w correction}\\
\end{tabular}
\caption{\label{fig:autocorrelationTIonly}\textbf{Comparing speckle auto-correlation in \AlgName with and without correction.} (a) Without correction, larger displacements at the outer image regions are degraded by the phase ramp. (b) After phase correction, {\AlgName} can clearly recover the auto-correlation.   }
\end{figure} 

==> figure/compare_algorithm_TI_only.tex <==
\begin{figure}[!t]
\centering
%\hspace{-1em}
\begin{tabular}{PP@{\hskip 1.8em}PP}
   \multicolumn{2}{c}{ \shifttext{-2em}{Full-frame}}  & \multicolumn{2}{c}{ \shifttext{-1em}{Local support}} \\ \cmidrule(r{1.2em}){1-2} \cmidrule{3-4}
 w/o correction & w correction &  w/o correction & w correction \\
\comparecorrectionlfsp{./figure/compare/collisionfree_ffrecon}{./figure/compare/collisionfree_recon} \\
\comparecorrectionlfsp{./figure/compare/fluorescent_ffrecon_redo}{./figure/compare/fluorescent_recon_redo}
\end{tabular}
\caption{\textbf{Comparing reconstruction in \AlgName with and without correction.} Top part: sparse, simple shifting laser target. Lower part: challenging fluorescent beads target. For the simple target on the top, the full-frame algorithm with correlation provided by {\AlgName} fails to recover all beads when excluding phase correction. The local correlation approach which is more robust to noise can recover the target even with the simpler modulations.  For the challenging target at the lower part, the full-frame algorithm fails completely even with phase correction. The local correlations algorithm can reconstruct the target using {\AlgName} modulations. However, without phase correction, it can only reconstruct a subset of the beads.}
\label{fig:compalgTIonly}
\end{figure} 
